Bandit Social Learning: Exploration under Myopic Behavior

We study social learning dynamics motivated by reviews on online platforms. The agents collectively follow a simple multi-armed bandit protocol, but each agent acts myopically, without regards to exploration. We allow the greedy (exploitation-only) algorithm, as well as a wide range of behavioral biases. Specifically, we allow myopic behaviors that are consistent with (parameterized) confidence intervals for the arms' expected rewards. We derive stark learning failures for any such behavior, and provide matching positive results. The learning-failure results extend to Bayesian agents and Bayesian bandit environments. In particular, we obtain general, quantitatively strong results on failure of the greedy bandit algorithm, both for ``frequentist" and ``Bayesian" versions. Failure results known previously are quantitatively weak, and either trivial or very specialized. Thus, we provide a theoretical foundation for designing non-trivial bandit algorithms, \ie algorithms that intentionally explore, which has been missing from the literature. Our general behavioral model can be interpreted as agents' optimism or pessimism. The matching positive results entail a maximal allowed amount of optimism. Moreover, we find that no amount of pessimism helps against the learning failures, whereas even a small-but-constant fraction of extreme optimists avoids the failures and leads to near-optimal regret rates.

==> app-K-proofs.tex <==
\section{Detailed proofs for $K$ arms}
\label{app:K-proofs}

In this appendix we provide full proofs for Section~\ref{sec:K}.

\subsection{Proof of Theorem~\ref{thm:K-LB}}

\subsection{Proof of Theorem~\ref{thm:K-LB-pess}}

\subsection{Proof of Theorem~\ref{thm:K-BG}} 

==> sec-IE.tex <==
\section{Implications for incentivized exploration}
\label{sec:IE}
